Infectious Disease Transmission via Aerosol Propagation from a Molecular Communication Perspective: Shannon Meets Coronavirus

Molecular communication is not only able to mimic biological and chemical communication mechanisms, but also provides a theoretical framework for viral infection processes. In this tutorial, aerosol and droplet transmission is modeled as a multiuser scenario with mobile nodes, related to broadcasting and relaying. In contrast to data communication systems, in the application of pathogen-laden aerosol transmission, mutual information between nodes should be minimized. Towards this goal, several countermeasures are reasoned. The findings are supported by experimental results and by an advanced particle simulation tool. This work is inspired by the recent outbreak of the coronavirus (COVID-19) pandemic, but also applicable to other airborne infectious diseases like influenza.

==> Commentary.tex <==
\section*{Letter to the Editor}

% The review of the above manuscript submitted to IEEE Communications Magazine has been completed. The reviewers have recommended that major revisions be made to the manuscript. An acceptance decision will not be made until these revisions have been made and a second review has been completed, and the manuscript may be rejected if these revisions are not made satisfactorily and in a timely manner.
\noindent\fbox{%
    \parbox{\linewidth}{%
        % {\textbf{Submission until 1st February 2021}}
        
        In the revised manuscript, we would like to remind you to ensure full compliance with all our format guidelines (https://www.comsoc.org/commag/manuscript-submission-guidelines), including, but not limited to, the following: 
        
        1) Maximum 7 pages (per the specifications described in the guidelines), 
        
        2) No Mathematical content unless approved by EiC (current knowledge of advanced mathematics should not be a requirement/condition for the reader to understand the paper), 
        
        3) Up to six figures and tables combined (manuscripts may not excessively include sub-figures and sub-tables to get around this guideline), 
        
        4) No more than fifteen (15) archival references that are complete with the publication name/title, year, volume, issue and page numbers. All references to online sources (website URLs, web-posted papers) are required to show an "Accessed on" date. All non-archival references (unpublished/to- be-published/pending/in-press-papers/reports) are required to show planned publication date, and volume/issue numbers. Otherwise, they are to be removed from the "References" section, and 
        
        5) a CrossChek Plagiarism Similarity Index that is less than 20%. 
    }%
}

% Every revision of the manuscript is expected to make considerable progress towards publication. Furthermore, if the manuscript fails to demonstrate considerable and steady progression towards publication, it may be rejected upon any revision. 

% Authors are required to submit revisions within certain period of time after which the manuscript can no longer be considered for publication and is withdrawn from the system:
% • Unless a shorter duration is required due to special editorial reason, an R1 must be submitted no later than forty five (45) days after R0 receives a revision decision.

% It is recommended that authors of a manuscript where revision was requested return a list of point-by-point responses to reviewers’ remarks. These responses must be included in a file separate from the revised manuscript. A standalone revised manuscript is always necessary to check format compliances.

% The reviewers' comments concerning the current version of your manuscripts are included below. **Please note-There may be files attached to the reviewer's comments. You will not be able to view attached files from this e-mail. To view attachments, please log into your Author Center and click on "View Letter" in the "Processing Status Column" of the table at the bottom of the page.

% Respond to the editor and reviewers by clicking on "View Comments/Respond" and entering responses in the appropriate fields. To upload a revision of your article, click on its title and follow the instructions. Be sure to complete all pages and click "continue" at the bottom of each one until the revised manuscript has been uploaded successfully.

% Once the article has been submitted you will receive an email stating that fact. If you do not receive an email to that effect, return to the author center at Manuscript Central and check to see if the article is listed in the Partially Submitted queue. If it is in this queue, you should complete the submission at that time. If you are unsure of how to proceed or you do not see your manuscript in the list of submitted or partially submitted articles, contact the administrator (tnkouatchah@gmail.com).

% Thank you for submitting your manuscript to IEEE Communications Magazine.

% NanoNetworking FT Editors

\vspace{5mm}
\textbf{Guest Editor: Editors, NanoNetworking FT}

Paper topic is timely and interesting.

{\color{blue} Many thanks for handling and supporting our manuscript.  We have put much effort in the mean time to include all constructive comments by you and the three reviewers in order to improve the manuscript.} 

However, following major issues should be handled with care:

- main contribution, i.e., using the mutual information for measuring the infection performance, should be highlighted and elaborated.

\begin{quote}
    \color{blue} Extensions regarding mutual information are mentioned in the feedback to Reviewer 1.
\end{quote}

- information about the simulation part is not adequate.

\begin{quote}
    \color{blue} Clarifications regarding the simulation part are mentioned in the feedback to Reviewers 1, 2, and 3.
\end{quote}

- linking with the Molecular communications is not detailed enough.

\begin{quote}
    \color{blue} The link to macro-scale molecular communications is pointed out in the feedback to Reviewer 1.\\ 
\end{quote}

\textbf{Reviewer: 1}

The authors propose to consider the aerosol propagation model of infectious diseases as an application of molecular communications. They represent each person in a closed environment as a communication node in a multi-user communications setup and discuss how people getting infected act as a relay that starts transmission.

The topic, due to the current pandemic, is obviously timely, but the I am not sure about what the contribution of this particular manuscript is. The content, including the model referenced in the above paragraph, generally read as a summary of the authors’ submitted work in [9].

\begin{quote}
    \color{blue}
    We would like to thank the reviewer for the fruitful comments and criticism, which helped us a lot in improving the paper. We have more clearly highlighted and elaborated on the points that set this paper apart from our previous publication. These include:
    \begin{itemize}
    \item The conceptual description of the duality between macro-scale MC and the spread of infectious diseases with emphasis on multiuser scenarios has been clarified. Details on the emission, propagation and reception of aerosols were further highlighted and expanded upon.
    \item The elaboration on the use of mutual information to determine the ``infection performance'' of air-borne diseases was extended. A simple example of channel modeling has been inserted in form of a figure.  As no formulas are allowed in this magazine paper, details and a critical review of this metric were collected in an arXiv paper. 
    \item Section~IV on advanced aerosol simulation has been rewritten.  The motivation for particle-based computer simulations is clarified, and a comparison with computational fluid dynamics is presented.  Possible extensions are given. 
    \item Section~V has been renamed in ``Prospects and Challenges''.  The text has been revised substantially.  
    \end{itemize}
\end{quote}

The numerical simulation results, again obtained from the same source as [9], show how particles originating from a simulated cough travel and land on the floor. This type of approach helps researchers model how far the social distancing needs to be maintained to avoid high risk zones, and has been done many times by many groups since the beginning of the pandemic, if not earlier. This type of work obviously needs a lot of assumptions from the user, such as the varying amount of viral load each individual is able to resist against (before being infected), how much delay occurs between reaching the viral load level and becoming infectious, and in what way secondary particles landing on for example hand are transported to the sensitive organs.

\begin{quote}
    \color{blue} In Section~IV, the paragraph on the pros and cons of the novel Pogona simulator and existing computational fluid dynamics (CFD) tools is revised considerably. Furthermore, a link to the  website of the Pogona simulation tool is added as a footnote:  https://www2.tkn.tu-berlin.de/software/pogona.  The software is optimized for particle transmission and downloadable for free. Physical-layer particle simulation tools are able to support simulation tools on networking layer.\\
    
    The motivation for computer simulations is revised as follows:
    
    ``To gain further insight into such multiuser scenarios as described above, computer simulations can be used. Compared to pure mathematical analysis, simulations afford flexibility in placing transmitters, receivers, and obstacles at arbitrary positions.  Simulations also offer expandability in keeping the door open for future implementations of additional physical phenomena such as Brownian motion or other mobility pattern.''\\
    
    The trade-off between particle simulation and CFD is explained as follows:
    
    ``Using a state of the art particle simulator (e.g., \cite{Schurwanz2020}), however, comes with a trade-off in physical accuracy as, for example, air movement and turbulence due to ventilation or convection is treated in an abstract way. In contrast, CFD helps to accurately assess the way in which infectious aerosols spread in an enclosed space (e.g., to investigate the effectiveness of ventilation).''\\
    
    Possible future developments are motivated as follows: 
    
    ``In future work, this simulation concept can be extended further to account for both the aspect of mobility and the remaining types of aerosol emissions outlined in Section~II. Mobility can be realized, for example, by letting simulated persons follow predetermined paths collected from mobility models or traces.  When incorporating other emission types, e.g., using the  air-based testbed outlined in Section~II, MoVCSK can be used as a modulation scheme to control the emission of particles.  In this context, it will also be important to support aerosol  particles with diameters smaller than \SI{50}{\micro\meter}.  Doing this accurately is difficult without  resorting to computation-intensive multiphysics and CFD simulations.  A sufficiently accurate  approximation could be obtained by expanding the original concept of the Pogona simulator \cite{drees2020efficient} and to guide aerosol particles through a sequence of samples of a time-varying pre-computed and locally constrained vector field.  Also, particle simulation tools could be used to support simulation tools on social (``networking'') layer.''
\end{quote}

I think the biggest contribution of the manuscript (again coming from [9]) is the promise of using mutual information to measure the "infection performance" of the virus. The manuscript does not move forward in this direction and leaves this as a thought. As Section V states, new findings from MC techniques can be used in infectiology, but this manuscript neither does this, nor provides a framework to demonstrate how it could be done.

\begin{quote}
    \color{blue} 
    In [9], mutual information is mentioned in a single sentence only: ``In other words, in data transmission a maximization of the mutual information is targeted, whereas in the case of virus transmission, a minimization of the mutual information is targeted.''
    
    Concerning mutual information, the current manuscript moves forward in two directions: Section~III~A provides an analogy between aerosol-based infection and mutual information; Section~III~B presents preventive approaches to reduce the mutual information.  
    
    In Section~III~A, the mathematical notations have been deleted as requested by Reviewer~2.  The text has been extended.  A supporting figure on channel modeling (Fig.~\ref{fig:z_channel}) has been added.  This figure depicts the input and transition probabilities, which form the basis for a calculation of mutual information and related infection measures.  The revised text is as follows: 
    
    {\color{blue} ``The mutual information of a point-to-point communication channel is determined by the distribution of the channel input events as well as by the transition probabilities between channel input and channel output events. In the scenario under investigation, the channel input distribution depends on the respiratory events. The transition probabilities depend on the statistics of the turbulent atmospheric channel, including receiver-side properties like the sensitive area \cite{Hoeher2021}. An intuitive example is shown in Fig.~\ref{fig:z_channel}.  Out of 10,000 emitted particles, 10~\% are infectious.  This stipulates the input distribution.  Just 50 of the 1,000 emitted infectious particles hit the sensitive area of the receiver, corresponding to a transition probability of 5~\%. This concept can be generalized to multipoint-to-multipoint channel models.  For details and a critical review of infection rate measures see \cite{Hoeher2021}.''}

    We agree that a more detailed framework regarding mutual information is desirable.  Due to the magazine-style constraints (strict page limitation, no equations) we have outsourced our thoughts in a separate paper entitled ``On Mutual Information Analysis of Infectious Disease Transmission via Particle Propagation.'' This paper is available at the arXiv online platform (arXiv preprint arXiv:2101.12121) and it is attached to this letter-to-the-editor.  A link is provided as reference \cite{Hoeher2021}.  The styles of the arXiv paper and this IEEE Communications Magazine manuscript are completely different and overlap has been avoided. 
    
    Section~III~B has been extended based on suggestions raised by Reviewers~2 and~3.
\end{quote}

In summary, although I enjoyed reading the manuscript (due to the -hopefully temporary- interest in the pandemic), I could not find any specific contributions beyond what was presented in [9]. Although the manuscript is meant to be a tutorial paper, I wasn't able to get much insight into the useful links between MC and infectious diseases beyond what is already discussed in many works in the past.

\begin{quote}
    \color{blue}
    The benefit of our contribution lies in the merging of insights from the fields of communication/ information theory and infectiology. By pointing out dualities, the similarities of the metrics become clear, which helps to provide a common framework and to widen the view.  Society would benefit from a better understanding of the spread of virus infections, not just Corona. Section~V has been revised considerably to emphasize on the prospects and challenges.\\ 
    
    To our best knowledge, at the time of submission previous works on the duality between molecular communication and pathogen-laden transmission have focused on point-to-point links, except our own contribution [9].  Unlike [9], this tutorial does not report about own human experiments. This tutorial presents the following communication aspects in greater depth: 
    \begin{itemize}
    \item The transmission of infectious particles is modeled as a multiuser MC scenario with mobile nodes in a time-varying environment. Infected users are transmitters that broadcast pathogen-laden particles, while the remaining users are potential receivers. After infection plus incubation times, some receivers may become  active transmitters, like in relaying. During this expected long delay, the environmental setup is likely to change completely.  
    
    Neither broadcasting nor relaying are mentioned in [9] as duality aspects linking MC with infection. 
    \item Infection is considered to be a generalized threshold detection problem: if the density of infectious particles received exceeds a user-dependent threshold, an infection is likely to occur. Furthermore, the viral load may also affect the course of the disease. In the field of MC, the corresponding analogy is reliability information.  
    
    According to the state of the art, hypothesis testing is performed, which corresponds to a hard decision.  This does not explain the course of the disease. 
    \item The viral infection rate is modeled by the concept of mutual information.  Contrary to data transmission, the aim is to minimize the mutual information between an infected user and the healthy ones.
    
    Mutual information as a measure of the infection rate is also an important link between MC and virus transmission.  The section on mutual information is extended in R1 as requested. 
    \end{itemize}
    
    The entire manuscript is revised carefully.\\
\end{quote}

\textbf{Reviewer: 2}

The article gives an overview of a new concept that studies infectious disease transmission via aerosol channels from a molecular communication point of view. This new perspective study is timely, exciting, and complements existing studies of virus detection. Additionally, this study is essential to analyze the effect of different infectious diseases transmission parameters and mitigation. Although the study’s value in this article, several aspects need further discussion and clarification or even included before considering this study. In the following, I list these aspects without a specific order:

\begin{quote}
    \color{blue}The authors thank the reviewer for this encouraging comment. 
\end{quote}

1) The authors should discuss the time scales associated with any study and classify it similar to the MC scale-based studies, which is either a microscopic or macroscopic scale. For example, in a small people gathering, the infection time can be in the order of minutes; however, the time required for such a human to become an active transmitter can be extended to days. In such cases, the system layout can change, including communication channels, number of transmitters, number of receivers, … etc.
Specifically, in the multiuser scenario subsection, the authors mentioned, “Those users can be modeled as store and forward relays, which after some delay may broadcast even more pathogens.” What is the range of delays? In case of an expected long delay, the setup may be completely changed.

\begin{quote}
    \color{blue} We thank the reviewer for asking for clarification regarding the time scale. In the introduction, our contribution is classified as MC on macroscopic scale.  Indeed, in MC on macroscopic scale, time scales can vary significantly.  The original wording ``after a certain delay'' is not precise.  We have meant the overall infection plus incubation time.  The introduction has been revised as follows: 
    
    ``After  infection  plus incubation  times,  some  of  the  receivers  may  become active transmitters, like in relaying. During this expected long  delay,  the  environmental  setup  is  likely  to  change completely.''
    
    Section~II was extended as follows:
    
    ``In  case  of  a  successful transmission  –  a  necessary  condition  is  that  the  ingested amount of infectious aerosols exceeds the infection threshold –the receiver itself becomes an active transmitter after infection plus incubation period. The infection time can be on the order of  minutes,  but  the  time  required  for  a  human  to  become  an active transmitter can be up to several days.'' 
    
    Also, ``relay'' has been expanded by ``agile relay'' in order to emphasize mobility. 
\end{quote}

2) As a result of the previous comment, the number of transmitters and the number of receivers tend to be discrete random variables. The point that should be included clarifying: when should we do so and what is the appropriate model?

\begin{quote}
    \color{blue} The reviewer is correct.  In Section~II~D we have added: 
    
    ``Accordingly, the number of transmitters is randomly distributed.'' 
    
    An appropriate analytical model for the number of active transmitters in a well-defined environment currently is unknown.  This is one of the reasons why we promote computer simulations, c.f.~Section~IV. 
\end{quote}

3) The authors mentioned: “Section II describes the duality between communication and information theory on the one hand and the field of airborne aerosol infection on the other.” My question/concern is: what is the position of molecular communication in this duality study? I believe

\begin{quote}
    \color{blue} We are sorry to say that in the review decision we have received by the Guest Editor the sentence stops after ``I believe''.  Therefore, we hope that we were able to interpret the question/concern correctly.  The questionable sentence has been changed: 
    
    ``Section~\ref{sec:scenario} describes the duality between MC (comprising communication and information theory) on the one hand and the field of airborne aerosol infection on the other.''
    
    From Table~I it is clear that duality aspects have been studied between MC on the one hand and infectious particle transmission on the other hand. Aspects developed by the communication and information theory community are subsumed in the interdisciplinary area of MC. 
\end{quote}

4) The authors wrote: “The particle clouds of different respiratory events superimpose.” My point is regarding superimpose, which refer to accumulation; however, this is not the general case because the particle clouds may react with each other. For example, the exhaled breath contains several volatile organic compounds, which may react with some particle clouds.

\begin{quote}
    \color{blue} Sorry about the confusion.  We did not had a linear superposition in mind.  The text has been rewritten as follows:
    
    ``The particle clouds of different respiratory events overlay and may react with each other. All parameters are of stochastic nature. The actual emitted aerosol distribution is user-dependent and may vary for each emission.  Larger droplets may shrink in dry air or split into smaller ones.''
\end{quote}

5) Further discussion should be added about emulating the infection process that transforms the receiver into a transmitter.

\begin{quote}
    \color{blue} The authors thank the reviewer for mentioning this aspect. We have deliberately avoided medical and biological details of the infection process within users. Furthermore, formulas are to be avoided in the magazine style.  A mathematical description on emulating the infection process is given in Equation~(10) of the new reference \cite{Hoeher2021}.  Classically, hypothesis testing is performed to transform a receiver into a transmitter as proposed in \cite{Khalid2020, Gulec2020}. 
\end{quote}

6) The relation of droplet size and gravity should be highlighted, where small droplets are subjected to negligible gravity force compared with the large ones. Also, the propagation distance will be affected.

\begin{quote}
    \color{blue} We thank the reviewer for this hint. We added a clarification in Section II to distinguish between aerosols and droplets:
    
    ``In the scenario under consideration, the signal strengths are defined by the parameters of the emitted aerosols and droplets by the different users. The term aerosols is used in the literature for various particles sizes between approximately $\SI{1}{\micro\meter}$ and several $\SI{1000}{\micro\meter}$. In this publication, aerosols describe the smaller particles that experience negligible influence from gravitational forces and droplets describe larger particles that are forced to the ground relatively quickly by gravitational forces.'' 
    
    In the Pogona simulation tool, the effect of the particle size on drag and gravity is considered. 
\end{quote}

7) The authors mentioned: “artificial air movement. The turbulent channel can be described by Shannon’s “mother of all models” [14]. This analogy is exploited subsequently.”
This discussion is not clear, where the well-known Shannon expression is for Gaussian noise and a given channel coefficient. Also, the connection with title is not clear: “Shannon Meets Coronavirus”.

\begin{quote}
    \color{blue} We are very sorry about this confusion.  Shannon's well-known expression for the channel capacity of the Gaussian channel should not be confused with his famous channel model depicted in Fig.~1 of his 1948 landmark paper.  This channel model, nowadays sometimes dubbed ``mother of all models'' (https://en.wikipedia.org/wiki/Shannon-Weaver\_model), comprises a source, a transmitter, a noisy channel, a receiver, and a sink.  Exactly this setup can be formulated in the context of particle transmission.  A connection to the Gaussian channel was not intended at this point.  In order to avoid any confusion, the corresponding paragraph has been deleted. 
    
    The subtitle ``Shannon Meets Coronavirus'' links the main title to Shannon's work.  As confirmed by the Guest Editor, mutual information is a core topic of our contribution.  Indeed, mutual information is the mathematical link between the different fields considered by Shannon.  As an honor, numerous authors have published papers with similar subtitles.  Particularly in magazine papers striking subtitles are not uncommon. 
\end{quote}

8) The emulation method in the multiuser scenario subsection does not seem to be practically proper. Indeed, more solid and accurate models and emulation techniques need to be considered.

\begin{quote}
    \color{blue} The text has been revised as follows: 
    
    ``In our testbed~\cite{Bhattacharjee2020a}, a point-to-multipoint scenario can be emulated by a network of pipelines with multiple camera receivers placed along their lengths with stationary or mobile sprayers releasing the water-based dye solution. If the intensities recorded by the cameras breach a certain threshold level, the receivers may be termed as ``infected'' actuating new sprayers after a certain delay, mimicking a relay mechanism.''
\end{quote}

9) The authors need to consider the initial condition status of the ambient air in their discussions.

\begin{quote}
    \color{blue} Thanks for this hint, we have added the following note to Section~II~C:
    
    ``Depending on the initial conditions in the environment, the range of the emitted aerosols can be influenced from the beginning.''
\end{quote}

10) The mathematical discussion in the mutual information subsection is not appropriate in magazine-style. It is recommended to omit it.

\begin{quote}
    \color{blue} Many thanks for this comment.  We have eliminated the mathematical notation. The text has been rewritten as follows and Fig.~\ref{fig:z_channel} has been added:
    
    ``The mutual information of a point-to-point communication channel is determined by the distribution of the channel input events as well as by the transition probabilities between channel input and channel output events. In the scenario under investigation, the channel input distribution depends on the respiratory events. The transition probabilities depend on the statistics of the turbulent atmospheric channel, including receiver-side properties like the sensitive area \cite{Hoeher2021}. An intuitive example is shown in Fig.~\ref{fig:z_channel}.  Out of 10,000 emitted particles, 10~\% are infectious.  This stipulates the input distribution.  Just 50 of the 1,000 emitted infectious particles hit the sensitive area of the receiver, corresponding to a transition probability of 5~\%.  This concept can be generalized to multipoint-to-multipoint channel models.  For details and a critical review of infection rate measures see \cite{Hoeher2021}. The analogy between aerosol-based infection and mutual information demonstrates three important facts: the risk of infection depends on the channel input distribution including number of events, the turbulent channel, and the infection threshold. Although a minimization of mutual information is counterproductive in classical communication scenarios, it is a common design objective in cryptosystems.''

    We should keep in mind that the Guest Editor requests to highlight and elaborate the main contribution, i.e., using the mutual information for measuring the infection performance.
\end{quote}

11) In the chemical-actions subsection, it is recommended to include a discussion related to disinfection and purifying sprays, which can eliminate the viruses in seconds and stays suspended in the air for minutes, killing other viruses.

\begin{quote}
   \color{blue} Many thanks for this hint.  The following sentence has been added:
    
    ``Disinfection and purifying sprays are a good alternative, as they can eliminate different kinds of viruses quickly. They might also stay suspended in air to further reduce the infectious particles over a longer period of time.''
    
    %\color{cyan} Remark by Sunasheer: Disinfectant fogging system has been used in pharmaceutical and food processing industries in the past for the decontamination of air mainly through dry vapor, micro-condensation and activated or ionized processes (Refer "COVID-19 in indoor environments — Air and surface disinfection measures").
\end{quote}

12) The “Advanced Aerosol Simulation” section is weak.
The authors need first to motivate using simulation rather than mathematical analysis.
Then, they need to discuss and refer to the theory behind computation methods.
After that, they should discuss the challenges in developing such simulations.
They should mention examples of complicated systems that need such computational fluid dynamics tools.
Another question, what about the existence of different airflows and turbulent sources.

\begin{quote}
    \color{blue} We thank the reviewer for this advice.
    We have added the following remarks to motivate the use of simulation in general:

    ``To gain further insight into such multiuser scenarios as described above, computer simulations can be used. Compared to pure mathematical analysis, simulations afford flexibility in placing transmitters, receivers, and obstacles at arbitrary positions. Simulations also offer expandability in keeping the door open for future implementations of additional physical phenomena such as Brownian motion or other mobility pattern.''

    For the theory behind the simulation methods used, we cite the Pogona simulator~\cite{drees2020efficient} and our previous publication~\cite{Schurwanz2020}, in which we discussed how the Pogona simulator was used to simulate particles expelled from a cough.

    The main challenge we see in these simulations is a trade-off between physical accuracy (computational fluid dynamics, slow) compared to our particle simulations.
    We added the following clarification:

    ``Using a state of the art particle simulator (e.g., \cite{Schurwanz2020}), however, comes with a trade-off in physical accuracy as, for example, air movement and turbulence due to ventilation or convection is treated in an abstract way. In contrast, CFD helps to accurately assess the way in which infectious aerosols spread in an enclosed space (e.g., to investigate the effectiveness of ventilation).''
    
    Additionally, the website of the Pogona simulation tool is added as a footnote: https://www2.tkn.tu-berlin.de/software/pogona/
\end{quote}

13) The “challenges and discussion” section is fragile and unacceptable. It is like a conclusion. Deep discussion regarding the challenges, solutions and opportunities must be included.

\begin{quote}
    
    \color{blue} This section was very weak indeed and has significantly been rewritten. This was all done under the premise of providing a discussion on possible uses and the advantages of the duality shown.
    
    ``Over time, much research has been done in the field of infection prevention. It is already possible to predict the course of infections in defined scenarios and to estimate the consequences of a certain number of infections. Techniques such as ``social distancing'' are results of this work.

    The use of mutual information as a measure of the infection rate provides a common framework for different areas including engineering and infectiology. Emphasis is on a conceptual level by pointing out dualities and similarities between these fields in order to widen the view. New findings from existing and refined MC techniques can be applied in infectiology and evaluated from a health care point of view.  These may include improved distance rules for certain situations or guidance on placing novel sensors. Under the premise of enabling everyone to ``live with the virus'' with as few restrictions as possible, it is desirable to adapt the infection control solutions more precisely to the circumstances in specific situations.

    Furthermore, a reverse check of established infection prevention techniques can be accomplished by means of tools established in communication and information theory.  Nevertheless, especially when combining different disciplines like engineering and health care, it should be checked whether the proposed approaches are fundamentally correct, which in turn might lead to new prevention approaches being useful in the real world and thus reducing the incidence of infection.

    Air-based MC offers new possibilities regarding the investigation of aerosol propagation. Testbeds and measurement tools can be used to verify precautions and to gain further insights into infection paths. Society would benefit from a better understanding of the spread of virus infections, not just Corona.''
\end{quote}

The authors need to address the aforementioned points in order to improve their study.

\begin{quote}
    \color{blue} The authors would like to thank the reviewer for the constructive comments.  All points have been addressed.\\ 
\end{quote}

\textbf{Reviewer: 3}

This paper studied aerosol transmission, propagation, and reception from the molecular communication perspective. The authors also interpreted infection prevention as a minimization of the mutual information between a transmitter and a receiver and reviewed six preventive approaches from the communication perspective. Overall, it is a hot topic and the paper is well written. My comments are as follows:

\begin{quote}
    \color{blue}The authors would like to thank the reviewer for this encouraging statement and the constructive comments. 
\end{quote}

1. Throughout the paper, aerosols and droplets are mentioned many times. Also, in Sec. II, the authors stated that aerosols would survive for a longer period than droplets in an environment. However, a clear definition and a comparison between aerosols and droplets are missing, which is difficult to follow for the members of the communication filed without MC background.

\begin{quote}
    \color{blue} We noticed that we were not clear about the use of the terms aerosols and droplets. We have therefore reviewed the usage throughout the paper and added a defining section:
    
    ``In the scenario under consideration, the signal strengths are defined by the parameters of the emitted aerosols and droplets by the different users. The term aerosols is used in the literature for various particles with sizes between approximately $\SI{1}{\micro\meter}$ and several $\SI{1000}{\micro\meter}$. In this publication, aerosols describe smaller particles that experience negligible influence from gravitational forces whereas droplets describe larger particles that are forced to the ground relatively quickly by gravitational forces.''

    % \color{magenta} Remark by Peter: There are two possible strategies solving this problem: 
    
    % 1) We may argue that in literature the term ``aerosol'' is used for a wide range of particle sizes (like we did in the introduction of the first paper).
    
    % 2) We may distinguish between aerosols and droplets.  As a general term, (airborne) particles could be used. 
\end{quote}

2. In Sec. III, the authors listed six preventive approaches to reduce the mutual information so as to reduce the risk of infection. Compared with other approaches/actions, the description of temporal actions is a little implicit. The authors are expected to use an example to explain this action. A scenario in my head is the departure lounge, but is it possible or feasible to allocate different time slots for passengers to talk?  

\begin{quote}
    \color{blue} 
    Silent periods in departure halls (and all other public areas) perhaps partially solve the problem, but shift work in office and industrial environments is more acceptable for many people, because it is common practice.  The text has been extended as follows: 
    
    ``\textit{Temporal actions:} The allocation of individual time slots on user or group level leads to a more orderly procedure and this results in a lower probability of infection. This technique is known as time-division multiple access and is widely used in communication engineering. Increasing the time between respiratory events reduces the likelihood of infection by pathogen-laden aerosols. An example is shift work.'' 
    
    %\color{cyan} Remark by Sunasheer: An example for temporal action would be for example, events like theatres and operas. Only a few people (performers) are given access to the channel in a timely fashion when they are singing, speaking, etc, while majority of the people (audience and other performers) remain silent and do not access the channel. This may be seen as TDMA in communication engineering. The probability of the spread of infection in this case is less as compared to an event such as a banquet with same number of people in the same location and space, where social interaction is maximum as everyone is talking to everyone simultaneously without any rules to accessing the channel in a timely fashion. \\  
    
    %\color{green!60!black} Remark by Martin: A concrete example is shift work in offices where employees are divided into groups and individual time slots in order to be able to maintain the distances to each other. In our case, for example, only one person may be in the office at a time, so one employee works, for example, in the morning and the other in the afternoon (TDMA). This is also common practice in industry.
\end{quote} 

3. From the description of the MC simulator in Sec. IV, it seems that in the authors’ simulator, they only simulate the propagation of particles.
However, the simulation of the aerosol emission (e.g., breathing, speaking/singing, and coughing/sneezing) and the aerosol reception are also very significant to study the whole communication system.
I guess that the simulation of emission and reception may rely on some molecular dynamics simulators, so a discussion of these simulators or others would complete this section.

\begin{quote}
    \color{blue}
    We added the following considerations to the end of Section~IV:\@

    ``In future work, this simulation concept can be extended further to account for both the aspect of mobility and the remaining types of aerosol emissions outlined in Section~II. Mobility can be realized, for example, by letting simulated persons follow predetermined paths collected from mobility models or traces.  When incorporating other emission types, e.g., using the  air-based testbed outlined in Section~II, MoVCSK can be used as a modulation scheme to control the emission of particles.  In this context, it will also be important to support aerosol  particles with diameters smaller than \SI{50}{\micro\meter}.  Doing this accurately is difficult without  resorting to computation-intensive multiphysics and CFD simulations.  A sufficiently accurate  approximation could be obtained by expanding the original concept of the Pogona simulator \cite{drees2020efficient} and to guide aerosol particles through a sequence of samples of a time-varying pre-computed and locally constrained vector field.  Also, particle simulation tools could be used to support simulation tools on social (``networking'') layer.''
\end{quote}
